A Convolutional Neural Network based Cascade Reconstruction for the IceCube Neutrino Observatory

Continued improvements on existing reconstruction methods are vital to the success of high-energy physics experiments, such as the IceCube Neutrino Observatory. In IceCube, further challenges arise as the detector is situated at the geographic South Pole where computational resources are limited. However, to perform real-time analyses and to issue alerts to telescopes around the world, powerful and fast reconstruction methods are desired. Deep neural networks can be extremely powerful, and their usage is computationally inexpensive once the networks are trained. These characteristics make a deep learning-based approach an excellent candidate for the application in IceCube. A reconstruction method based on convolutional architectures and hexagonally shaped kernels is presented. The presented method is robust towards systematic uncertainties in the simulation and has been tested on experimental data. In comparison to standard reconstruction methods in IceCube, it can improve upon the reconstruction accuracy, while reducing the time necessary to run the reconstruction by two to three orders of magnitude.

==> Makefile <==
target = dnn_reco_paper
all: build/$(target).pdf

texoptions = \
	     --pdf \
	     --interaction=nonstopmode \
	     --halt-on-error \
	     --output-directory=build

build/$(target).pdf: FORCE | build
	latexmk $(texoptions) $(target)

preview: FORCE | build
	latexmk $(texoptions) -pvc $(target)

FORCE:

build:
	mkdir -p build

clean:
	rm -r build


==> chapters/00_authors_old.tex <==
% \documentclass[preprint,12pt]{article}
% \usepackage{jheppub}
% \usepackage[T5,T1]{fontenc}
% \title{IceCube Author List for JHEP/JCAP 20201221}
%

\author[16]{R. Abbasi,}
\author[56]{M. Ackermann,}
\author[17]{J. Adams,}
\author[11]{J. A. Aguilar,}
\author[21]{M. Ahlers,}
\author[47]{M. Ahrens,}
\author[27]{C. Alispach,}
\author[30]{A. A. Alves Jr.,}
\author[40]{N. M. Amin,}
\author[13]{R. An,}
\author[38]{K. Andeen,}
\author[53]{T. Anderson,}
\author[11]{I. Ansseau,}
\author[25]{G. Anton,}
\author[13]{C. Arg{\"u}elles,}
\author[14]{S. Axani,}
\author[44]{X. Bai,}
\author[36]{A. Balagopal V.,}
\author[27]{A. Barbano,}
\author[29]{S. W. Barwick,}
\author[56]{B. Bastian,}
\author[36]{V. Basu,}
\author[37]{V. Baum,}
\author[11]{S. Baur,}
\author[7]{R. Bay,}
\author[19,20]{J. J. Beatty,}
\author[55]{K.-H. Becker,}
\author[10]{J. Becker Tjus,}
\author[26]{C. Bellenghi,}
\author[46]{S. BenZvi,}
\author[18]{D. Berley,}
\author[56,a]{E. Bernardini,}
\author[31,b]{D. Z. Besson,}
\author[7,8]{G. Binder,}
\author[55]{D. Bindig,}
\author[18]{E. Blaufuss,}
\author[56]{S. Blot,}
\author[37]{S. B{\"o}ser,}
\author[54]{O. Botner,}
\author[0]{J. B{\"o}ttcher,}
\author[21]{E. Bourbeau,}
\author[36]{J. Bourbeau,}
\author[56]{F. Bradascio,}
\author[36]{J. Braun,}
\author[27]{S. Bron,}
\author[56]{J. Brostean-Kaiser,}
\author[54]{A. Burgman,}
\author[39]{R. S. Busse,}
\author[43]{M. A. Campana,}
\author[5]{C. Chen,}
\author[36]{D. Chirkin,}
\author[49]{S. Choi,}
\author[23]{B. A. Clark,}
\author[32]{K. Clark,}
\author[39]{L. Classen,}
\author[40]{A. Coleman,}
\author[14]{G. H. Collin,}
\author[14]{J. M. Conrad,}
\author[12]{P. Coppin,}
\author[12]{P. Correa,}
\author[52,53]{D. F. Cowen,}
\author[46]{R. Cross,}
\author[5]{P. Dave,}
\author[12]{C. De Clercq,}
\author[53]{J. J. DeLaunay,}
\author[40]{H. Dembinski,}
\author[47]{K. Deoskar,}
\author[28]{S. De Ridder,}
\author[36]{A. Desai,}
\author[36]{P. Desiati,}
\author[12]{K. D. de Vries,}
\author[12]{G. de Wasseige,}
\author[9]{M. de With,}
\author[23]{T. DeYoung,}
\author[0]{S. Dharani,}
\author[14]{A. Diaz,}
\author[36]{J. C. D{\'\i}az-V{\'e}lez,}
\author[30]{H. Dujmovic,}
\author[53]{M. Dunkman,}
\author[36]{M. A. DuVernois,}
\author[44]{E. Dvorak,}
\author[37]{T. Ehrhardt,}
\author[26]{P. Eller,}
\author[30]{R. Engel,}
\author[18]{J. Evans,}
\author[40]{P. A. Evenson,}
\author[36]{S. Fahey,}
\author[6]{A. R. Fazely,}
\author[25]{S. Fiedlschuster,}
\author[53]{A.T. Fienberg,}
\author[7]{K. Filimonov,}
\author[47]{C. Finley,}
\author[56]{L. Fischer,}
\author[52]{D. Fox,}
\author[10,56]{A. Franckowiak,}
\author[18]{E. Friedman,}
\author[37]{A. Fritz,}
\author[0]{P. F{\"u}rst,}
\author[40]{T. K. Gaisser,}
\author[35]{J. Gallagher,}
\author[0]{E. Ganster,}
\author[56]{S. Garrappa,}
\author[8]{L. Gerhardt,}
\author[51]{A. Ghadimi,}
\author[54]{C. Glaser,}
\author[26]{T. Glauch,}
\author[25]{T. Gl{\"u}senkamp,}
\author[8]{A. Goldschmidt,}
\author[40]{J. G. Gonzalez,}
\author[51]{S. Goswami,}
\author[23]{D. Grant,}
\author[53]{T. Gr{\'e}goire,}
\author[36]{Z. Griffith,}
\author[46]{S. Griswold,}
\author[10]{M. G{\"u}nd{\"u}z,}
\author[26]{C. Haack,}
\author[54]{A. Hallgren,}
\author[23]{R. Halliday,}
\author[0]{L. Halve,}
\author[36]{F. Halzen,}
\author[26]{M. Ha Minh,}
\author[36]{K. Hanson,}
\author[36]{J. Hardin,}
\author[23]{A. A. Harnisch,}
\author[30]{A. Haungs,}
\author[0]{S. Hauser,}
\author[9]{D. Hebecker,}
\author[55]{K. Helbing,}
\author[26]{F. Henningsen,}
\author[23]{E. C. Hettinger,}
\author[55]{S. Hickford,}
\author[24]{J. Hignight,}
\author[15]{C. Hill,}
\author[1]{G. C. Hill,}
\author[18]{K. D. Hoffman,}
\author[55]{R. Hoffmann,}
\author[22]{T. Hoinka,}
\author[36]{B. Hokanson-Fasig,}
\author[36,c]{K. Hoshina,}
\author[53]{F. Huang,}
\author[26]{M. Huber,}
\author[30]{T. Huber,}
\author[47]{K. Hultqvist,}
\author[22]{M. H{\"u}nnefeld,}
\author[36]{R. Hussain,}
\author[49]{S. In,}
\author[11]{N. Iovine,}
\author[15]{A. Ishihara,}
\author[47]{M. Jansson,}
\author[4]{G. S. Japaridze,}
\author[49]{M. Jeong,}
\author[3]{B. J. P. Jones,}
\author[0]{R. Joppe,}
\author[30]{D. Kang,}
\author[49]{W. Kang,}
\author[43]{X. Kang,}
\author[39]{A. Kappes,}
\author[37]{D. Kappesser,}
\author[56]{T. Karg,}
\author[26]{M. Karl,}
\author[36]{A. Karle,}
\author[25]{U. Katz,}
\author[36]{M. Kauer,}
\author[0]{M. Kellermann,}
\author[36]{J. L. Kelley,}
\author[53]{A. Kheirandish,}
\author[49]{J. Kim,}
\author[15]{K. Kin,}
\author[56]{T. Kintscher,}
\author[48]{J. Kiryluk,}
\author[7,8]{S. R. Klein,}
\author[40]{R. Koirala,}
\author[9]{H. Kolanoski,}
\author[37]{L. K{\"o}pke,}
\author[23]{C. Kopper,}
\author[51]{S. Kopper,}
\author[21]{D. J. Koskinen,}
\author[30]{P. Koundal,}
\author[43]{M. Kovacevich,}
\author[9,56]{M. Kowalski,}
\author[26]{K. Krings,}
\author[37]{G. Kr{\"u}ckl,}
\author[43]{N. Kurahashi,}
\author[1]{A. Kyriacou,}
\author[56]{C. Lagunas Gualda,}
\author[53]{J. L. Lanfranchi,}
\author[18]{M. J. Larson,}
\author[55]{F. Lauber,}
\author[13,36]{J. P. Lazar,}
\author[36]{K. Leonard,}
\author[30]{A. Leszczy{\'n}ska,}
\author[53]{Y. Li,}
\author[36]{Q. R. Liu,}
\author[37]{E. Lohfink,}
\author[39]{C. J. Lozano Mariscal,}
\author[15]{L. Lu,}
\author[27]{F. Lucarelli,}
\author[23,33]{A. Ludwig,}
\author[36]{W. Luszczak,}
\author[7,8]{Y. Lyu,}
\author[56]{W. Y. Ma,}
\author[36]{J. Madsen,}
\author[23]{K. B. M. Mahn,}
\author[36]{Y. Makino,}
\author[0]{P. Mallik,}
\author[36]{S. Mancina,}
\author[11]{I. C. Mari{\c{s}},}
\author[41]{R. Maruyama,}
\author[15]{K. Mase,}
\author[34]{F. McNally,}
\author[36]{K. Meagher,}
\author[20]{A. Medina,}
\author[15]{M. Meier,}
\author[26]{S. Meighen-Berger,}
\author[0]{J. Merz,}
\author[23]{J. Micallef,}
\author[11]{D. Mockler,}
\author[37]{G. Moment{\'e},}
\author[27]{T. Montaruli,}
\author[24]{R. W. Moore,}
\author[57]{K. Morik,}
\author[36]{R. Morse,}
\author[14]{M. Moulai,}
\author[56]{R. Naab,}
\author[15]{R. Nagai,}
\author[55]{U. Naumann,}
\author[56]{J. Necker,}
\author[23]{L. V. Nguy{\~{\^{{e}}}}n,}
\author[26]{H. Niederhausen,}
\author[23]{M. U. Nisa,}
\author[23]{S. C. Nowicki,}
\author[8]{D. R. Nygren,}
\author[55]{A. Obertacke Pollmann,}
\author[30]{M. Oehler,}
\author[18]{A. Olivas,}
\author[54]{E. O'Sullivan,}
\author[40]{H. Pandya,}
\author[53]{D. V. Pankova,}
\author[36]{N. Park,}
\author[3]{G. K. Parker,}
\author[40]{E. N. Paudel,}
\author[37]{P. Peiffer,}
\author[54]{C. P{\'e}rez de los Heros,}
\author[0]{S. Philippen,}
\author[22]{D. Pieloth,}
\author[55]{S. Pieper,}
\author[36]{A. Pizzuto,}
\author[38]{M. Plum,}
\author[0]{Y. Popovych,}
\author[28]{A. Porcelli,}
\author[36]{M. Prado Rodriguez,}
\author[7]{P. B. Price,}
\author[23]{B. Pries,}
\author[8]{G. T. Przybylski,}
\author[11]{C. Raab,}
\author[17]{A. Raissi,}
\author[21]{M. Rameez,}
\author[2]{K. Rawlins,}
\author[26]{I. C. Rea,}
\author[40]{A. Rehman,}
\author[0]{R. Reimann,}
\author[30]{M. Renschler,}
\author[11]{G. Renzi,}
\author[26]{E. Resconi,}
\author[56]{S. Reusch,}
\author[22]{W. Rhode,}
\author[43]{M. Richman,}
\author[36]{B. Riedel,}
\author[7,8]{S. Robertson,}
\author[49]{G. Roellinghoff,}
\author[0]{M. Rongen,}
\author[49]{C. Rott,}
\author[22]{T. Ruhe,}
\author[28]{D. Ryckbosch,}
\author[23]{D. Rysewyk Cantu,}
\author[13,36]{I. Safa,}
\author[23]{S. E. Sanchez Herrera,}
\author[22]{A. Sandrock,}
\author[37]{J. Sandroos,}
\author[51]{M. Santander,}
\author[42]{S. Sarkar,}
\author[24]{S. Sarkar,}
\author[56]{K. Satalecka,}
\author[0]{M. Scharf,}
\author[0]{M. Schaufel,}
\author[30]{H. Schieler,}
\author[22]{P. Schlunder,}
\author[18]{T. Schmidt,}
\author[36]{A. Schneider,}
\author[25]{J. Schneider,}
\author[30,40]{F. G. Schr{\"o}der,}
\author[0]{L. Schumacher,}
\author[43]{S. Sclafani,}
\author[40]{D. Seckel,}
\author[45]{S. Seunarine,}
\author[54]{A. Sharma,}
\author[0]{S. Shefali,}
\author[36]{M. Silva,}
\author[13]{B. Skrzypek,}
\author[3]{B. Smithers,}
\author[36]{R. Snihur,}
\author[22]{J. Soedingrekso,}
\author[40]{D. Soldin,}
\author[45]{G. M. Spiczak,}
\author[56,b]{C. Spiering,}
\author[56]{J. Stachurska,}
\author[20]{M. Stamatikos,}
\author[40]{T. Stanev,}
\author[56]{R. Stein,}
\author[0]{J. Stettner,}
\author[37]{A. Steuer,}
\author[8]{T. Stezelberger,}
\author[8]{R. G. Stokstad,}
\author[21]{T. Stuttard,}
\author[18]{G. W. Sullivan,}
\author[5]{I. Taboada,}
\author[10]{F. Tenholt,}
\author[6]{S. Ter-Antonyan,}
\author[40]{S. Tilav,}
\author[0]{F. Tischbein,}
\author[23]{K. Tollefson,}
\author[10]{L. Tomankova,}
\author[50]{C. T{\"o}nnis,}
\author[11]{S. Toscano,}
\author[36]{D. Tosi,}
\author[56]{A. Trettin,}
\author[25]{M. Tselengidou,}
\author[5]{C. F. Tung,}
\author[26]{A. Turcati,}
\author[30]{R. Turcotte,}
\author[53]{C. F. Turley,}
\author[23]{J. P. Twagirayezu,}
\author[36]{B. Ty,}
\author[39]{M. A. Unland Elorrieta,}
\author[54]{N. Valtonen-Mattila,}
\author[36]{J. Vandenbroucke,}
\author[36]{D. van Eijk,}
\author[12]{N. van Eijndhoven,}
\author[14]{D. Vannerom,}
\author[56]{J. van Santen,}
\author[28]{S. Verpoest,}
\author[28]{M. Vraeghe,}
\author[47]{C. Walck,}
\author[1]{A. Wallace,}
\author[3]{T. B. Watson,}
\author[23]{C. Weaver,}
\author[30]{A. Weindl,}
\author[53]{M. J. Weiss,}
\author[37]{J. Weldert,}
\author[36]{C. Wendt,}
\author[22]{J. Werthebach,}
\author[30]{M. Weyrauch,}
\author[1]{B. J. Whelan,}
\author[23,33]{N. Whitehorn,}
\author[37]{K. Wiebe,}
\author[0]{C. H. Wiebusch,}
\author[51]{D. R. Williams,}
\author[26]{M. Wolf,}
\author[7]{K. Woschnagg,}
\author[25]{G. Wrede,}
\author[10]{J. Wulff,}
\author[6]{X. W. Xu,}
\author[48]{Y. Xu,}
\author[24]{J. P. Yanez,}
\author[15]{S. Yoshida,}
\author[36]{T. Yuan}
\author[48]{and Z. Zhang}
\affiliation[0]{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\affiliation[1]{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\affiliation[2]{Dept. of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA}
\affiliation[3]{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\affiliation[4]{CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA}
\affiliation[5]{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\affiliation[6]{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}
\affiliation[7]{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation[8]{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\affiliation[9]{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\affiliation[10]{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\affiliation[11]{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\affiliation[12]{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\affiliation[13]{Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge, MA 02138, USA}
\affiliation[14]{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation[15]{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\affiliation[16]{Department of Physics, Loyola University Chicago, Chicago, IL 60660, USA}
\affiliation[17]{Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand}
\affiliation[18]{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\affiliation[19]{Dept. of Astronomy, Ohio State University, Columbus, OH 43210, USA}
\affiliation[20]{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}
\affiliation[21]{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\affiliation[22]{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\affiliation[23]{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\affiliation[24]{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\affiliation[25]{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\affiliation[26]{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\affiliation[27]{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\affiliation[28]{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\affiliation[29]{Dept. of Physics and Astronomy, University of California, Irvine, CA 92697, USA}
\affiliation[30]{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\affiliation[31]{Dept. of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}
\affiliation[32]{SNOLAB, 1039 Regional Road 24, Creighton Mine 9, Lively, ON, Canada P3Y 1N2}
\affiliation[33]{Department of Physics and Astronomy, UCLA, Los Angeles, CA 90095, USA}
\affiliation[34]{Department of Physics, Mercer University, Macon, GA 31207-0001, USA}
\affiliation[35]{Dept. of Astronomy, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\affiliation[36]{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\affiliation[37]{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\affiliation[38]{Department of Physics, Marquette University, Milwaukee, WI, 53201, USA}
\affiliation[39]{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\affiliation[40]{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\affiliation[41]{Dept. of Physics, Yale University, New Haven, CT 06520, USA}
\affiliation[42]{Dept. of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, UK}
\affiliation[43]{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\affiliation[44]{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\affiliation[45]{Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA}
\affiliation[46]{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}
\affiliation[47]{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\affiliation[48]{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}
\affiliation[49]{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\affiliation[50]{Institute of Basic Science, Sungkyunkwan University, Suwon 16419, Korea}
\affiliation[51]{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\affiliation[52]{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation[53]{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation[54]{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\affiliation[55]{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\affiliation[56]{DESY, D-15738 Zeuthen, Germany}
\affiliation[57]{Dept. of Computer Science, TU Dortmund University, D-44221 Dortmund, Germany} % Modification for Katharina
\affiliation[a]{also at Universit{\`a} di Padova, I-35131 Padova, Italy}
\affiliation[b]{also at National Research Nuclear University, Moscow Engineering Physics Institute (MEPhI), Moscow 115409, Russia}
\affiliation[c]{also at Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan}

%
% \begin{document}
% \maketitle
% \acknowledgments
% USA {\textendash} U.S. National Science Foundation-Office of Polar Programs,
% U.S. National Science Foundation-Physics Division,
% Wisconsin Alumni Research Foundation,
% Center for High Throughput Computing (CHTC) at the University of Wisconsin{\textendash}Madison,
% Open Science Grid (OSG),
% Extreme Science and Engineering Discovery Environment (XSEDE),
% Frontera computing project at the Texas Advanced Computing Center,
% U.S. Department of Energy-National Energy Research Scientific Computing Center,
% Particle astrophysics research computing center at the University of Maryland,
% Institute for Cyber-Enabled Research at Michigan State University,
% and Astroparticle physics computational facility at Marquette University;
% Belgium {\textendash} Funds for Scientific Research (FRS-FNRS and FWO),
% FWO Odysseus and Big Science programmes,
% and Belgian Federal Science Policy Office (Belspo);
% Germany {\textendash} Bundesministerium f{\"u}r Bildung und Forschung (BMBF),
% Deutsche Forschungsgemeinschaft (DFG),
% Helmholtz Alliance for Astroparticle Physics (HAP),
% Initiative and Networking Fund of the Helmholtz Association,
% Deutsches Elektronen Synchrotron (DESY),
% and High Performance Computing cluster of the RWTH Aachen;
% Sweden {\textendash} Swedish Research Council,
% Swedish Polar Research Secretariat,
% Swedish National Infrastructure for Computing (SNIC),
% and Knut and Alice Wallenberg Foundation;
% Australia {\textendash} Australian Research Council;
% Canada {\textendash} Natural Sciences and Engineering Research Council of Canada,
% Calcul Qu{\'e}bec, Compute Ontario, Canada Foundation for Innovation, WestGrid, and Compute Canada;
% Denmark {\textendash} Villum Fonden and Carlsberg Foundation;
% New Zealand {\textendash} Marsden Fund;
% Japan {\textendash} Japan Society for Promotion of Science (JSPS)
% and Institute for Global Prominent Research (IGPR) of Chiba University;
% Korea {\textendash} National Research Foundation of Korea (NRF);
% Switzerland {\textendash} Swiss National Science Foundation (SNSF);
% United Kingdom {\textendash} Department of Physics, University of Oxford.
% \end{document}


==> plots/data_mc/data_mc_feature_importance_table_cnn.tex <==
\begin{center}
	\begin{tabular}{ll}
		\toprule
		Feature Name & Importance \\
		\midrule
		CNN - Zenith & $0.18\pm0.17$ \\
		CNN - Energy & $0.17\pm0.16$ \\
		CNN - Azimuth & $0.17\pm0.16$ \\
		\bottomrule
	\end{tabular}
\end{center}


==> plots/data_mc/data_mc_feature_importance_table_combined.tex <==
\begin{center}
	\begin{tabular}{ll}
		\toprule
		Feature Name & Importance \\
		\midrule
		Standard - Zenith & $0.07\pm0.06$ \\
		CNN - Energy Unc. & $0.06\pm0.06$ \\
		CNN - Zenith & $0.06\pm0.06$ \\
		CNN - Azimuth & $0.06\pm0.05$ \\
		Standard - Azimuth & $0.06\pm0.05$ \\
		CNN - Azimuth Unc. & $0.06\pm0.05$ \\
		CNN - Zenith Unc. & $0.06\pm0.05$ \\
		Standard - Energy & $0.05\pm0.05$ \\
		CNN - Energy & $0.05\pm0.05$ \\
		\bottomrule
	\end{tabular}
\end{center}


==> plots/data_mc/data_mc_feature_importance_table_mle.tex <==
\begin{center}
	\begin{tabular}{ll}
		\toprule
		Feature Name & Importance \\
		\midrule
		Standard - Zenith & $0.17\pm0.17$ \\
		Standard - Azimuth & $0.17\pm0.16$ \\
		Standard - Energy & $0.16\pm0.16$ \\
		\bottomrule
	\end{tabular}
\end{center}


==> plots/data_mc/data_mc_feature_importance_table_test.tex <==
\begin{center}
	\begin{tabular}{ll}
		\toprule
		Feature Name & Importance \\
		\midrule
		$\mathrm{Var}_{x, c=0.9}$ & $0.09\pm0.07$ \\
		$\mathrm{Var}_{y, c=0.9}$ & $0.08\pm0.07$ \\
		$\mathrm{Var}_{x, c=0.5}$ & $0.06\pm0.05$ \\
		$\mathrm{Var}_{y, c=0.5}$ & $0.05\pm0.04$ \\
		$\mathrm{Var}_{y, c=0.0}$ & $0.03\pm0.02$ \\
		CNN - Zenith & $0.03\pm0.02$ \\
		Standard - Zenith & $0.03\pm0.02$ \\
		CNN - Energy Unc. & $0.03\pm0.02$ \\
		Standard - Energy & $0.02\pm0.02$ \\
		CNN - Azimuth Unc. & $0.02\pm0.02$ \\
		CNN - Energy & $0.02\pm0.02$ \\
		$\mathrm{Var}_{x, c=0.0}$ & $0.02\pm0.02$ \\
		CNN - Azimuth & $0.02\pm0.02$ \\
		CNN - Zenith Unc. & $0.02\pm0.02$ \\
		Standard - Azimuth & $0.02\pm0.02$ \\
		\bottomrule
	\end{tabular}
\end{center}

